Modeling and Control of an Omnidirectional Micro Aerial Vehicle Equipped with a Soft Robotic Arm

Flying manipulators are aerial drones with attached rigid-bodied robotic arms and belong to the latest and most actively developed research areas in robotics. The rigid nature of these arms often lack compliance, flexibility, and smoothness in movement. This work proposes to use a soft-bodied robotic arm attached to an omnidirectional micro aerial vehicle (OMAV) to leverage the compliant and flexible behavior of the arm, while remaining maneuverable and dynamic thanks to the omnidirectional drone as the floating base. The unification of the arm with the drone poses challenges in the modeling and control of such a combined platform; these challenges are addressed with this work. We propose a unified model for the flying manipulator based on three modeling principles: the Piecewise Constant Curvature (PCC) and Augmented Rigid Body Model (ARBM) hypotheses for modeling soft continuum robots and a floating-base approach borrowed from the traditional rigid-body robotics literature. To demonstrate the validity and usefulness of this parametrisation, a hierarchical model-based feedback controller is implemented. The controller is verified and evaluated in simulation on various dynamical tasks, where the nullspace motions, disturbance recovery, and trajectory tracking capabilities of the platform are examined and validated. The soft flying manipulator platform could open new application fields in aerial construction, goods delivery, human assistance, maintenance, and warehouse automation.

==> 02_model.tex <==
%
%
%
%%% Model
\section{Model} 
In this section, we propose a framework for modeling the dynamics of soft robots, linking it to an equivalent rigid robot constrained through a set of nonlinear integrable constraints. The key property of the model is to define a perfect matching under the hypothesis of piecewise constant curvature, enabling the application of control strategies typically used in rigid robots onto soft robots. 
%
%We first introduce the kinematics including an augmented formulation. Leveraging the augmented formulation, we describe the dynamic model and its properties.

\subsection{Kinematics}
\label{sec:kinematics}

In the Piecewise Constant Curvature (PCC) model, the infinite dimensionality of the soft robot's configuration is resolved by considering the robot's shape as composed of a fixed number of segments with constant curvature (CC), merged such that the resulting curve is everywhere differentiable. 
%
Consider a PCC soft robot composed by $n$ CC segments, and consider a set of reference systems $\{S_0\},\dots,\{S_n\}$ attached at the ends of each segment. Fig.~\ref{fig:PCC_ex} presents an example of a soft robot composed by four CC segments.
%
\begin{figure}
	\centering
    \includegraphics[width = .6\columnwidth]{dwg/PCC}
    \caption{Example of a Piecewise Constant Curvature robot, composed by four constant curvature elements. $\{S_0\}$ is the robot's base frame. A reference frame $\{S_i\}$ is connected at the end of each segment. $T_{i-1}^i$ is the homogeneous transformation mapping $\{S_{i - 1}\}$ into $\{S_i\}$.}
\end{figure}
%
Using the constant curvature hypothesis, ${S_{i-1}}$ and ${S_{i}}$ fully define the configuration of the $i\--th$ segment.
%
Thus, the robot's kinematics can be defined by $n$ homogeneous transformations $T_{0}^1,\dots,T_{n-1}^n$, which map each reference system to the subsequent one. 

In the interest of conciseness, we will consider the planar case. Please refer to \cite{webster2010design} for more details about the PCC kinematics in 3D case.
%
\begin{figure}
  \centering
  \includegraphics[width = .85\columnwidth]{dwg/segment_c.png}
  \caption{Kinematic representation of the i\--th planar constant curvature segment. Two local frames are placed at the two ends of the segment, $\{S_{i-1}\}$ and $\{S_{i}\}$ respectively. The length of the segment is $L_i$, and $q_i$ is the degree of curvature. \label{fig:CC_seg}}
\end{figure}
%
Fig.~\ref{fig:CC_seg} shows the kinematics of a single CC segment. Under the hypothesis of non-extensibility, one variable is sufficient to describe the segment's configuration. We use the relative rotation between the two reference systems, called the degree of curvature, as the configuration variable. Let us call this variable $q_i$ for the $i\--th$ segment. Then, the $i\--th$ homogeneous transformation can be derived using geometrical considerations as
%
\begin{equation} \label{eq:T}
	T_{i-1}^i(q_i) = 
    \begin{bmatrix}
		\cos(q_i) &-\sin(q_i) &L_i\frac{\sin(q_i)}{q_i} \\
        \sin(q_i) &\cos(q_i) &L_i\frac{1 - \cos(q_i)}{q_i} \\
        0 &0 &1 \\
	\end{bmatrix} \; ,
\end{equation}
%
where $L_i$ is the length of a segment. 
% Note, that for $q_i \rightarrow 0$, the transformation becomes 
% %
% \begin{equation}
% 	T_{i-1}^i(0) = \lim_{q_i \rightarrow 0}T_{i-1}^i(q_i) =
%     \begin{bmatrix}
% 		1 &0 &L_i \\
%         0 &1 &0\\
%         0 &0 &1 \\
% 	\end{bmatrix} \, .
% \end{equation}

\subsection{Dynamically-Consistent Augmented Formulation}
\label{sec:augmented}

An equivalent formulation of Eq.~\eqref{eq:T} in terms of elemental Denavit-Hartenberg (DH) transformations is introduced in \cite{hannan2003kinematics}. 
%Table~\ref{tab:DH1} presents one example, where Eq.~\eqref{eq:T} is realized as a sequence of two rotations (R) and a translation (P) along the $z$ axis. 
The framework we propose in this section leverages the intuition that such equivalence implicitly defines a connection between a soft robot and a rigid robot described by the equivalent DH-parametrization. Fig.~\ref{fig:augmented_robots} shows an example of robotic structures (an RPR robot) matching a single CC segment. More complex rigid structures matching a generic PCC soft robot can be built by connecting such basic elements.

% \begin{table}[ht]
% %\normalsize
% \centering 
% \caption{RPR Denavit-Hartenberg description of a single planar segment with constant curvature. \label{tab:DH1}}
% \begin{tabular}{ccccc}
% \hline
% Link &$\theta$ &d &a &$\alpha$  \\
% \hline
% $1$      &$\dfrac{q_i}{2}$  &0                                              &0 &$\dfrac{\pi}{2}$      \\
% $2$      &$0$                 &$2 \, L_i \, \dfrac{\sin(\frac{q_i}{2})}{q_i}$ &0 &$-\dfrac{\pi}{2}$      \\
% $3$      &$\dfrac{q_i}{2}$                 &$0$ &0 &$0$     \\
% \hline
% \end{tabular}
% \end{table}

We will refer to the state space of the equivalent rigid robot as the \textit{augmented state representation} of the PCC soft robot. We call $\xi \in \mathbb{R}^{n\,m}$ the augmented configuration, where $m$ is the number of joints per CC segment and $n$ is the number of segments. The two configurations are connected through the continuously differentiable map
%
\begin{equation}
	m: \mathbb{R}^{n} \rightarrow \mathbb{R}^{n\,m} \, .
\end{equation}
%
The map $\xi = m(q)$ assures that the end points of each CC segment coincide with the corresponding reference points of the rigid robot. 
% For the robot described by Table~\ref{tab:DH1}, the map is
% %
% \begin{equation}\label{eq:m_k}
% 	m_i(q_i) = 
% 	\begin{bmatrix}
% 		\frac{q_i}{2}\\
% 		2 \, L_i \frac{\sin(\frac{q_i}{2})}{q_i} \\
% 		\frac{q_i}{2}
% 	\end{bmatrix} \; .
% \end{equation}
% %
Note that from a kinematic point of view, any augment representation satisfying this condition is equivalent. %, as shown in Fig.~\ref{fig:augmented_robots}. 
However, as soon as we consider the dynamics of the two robots, another constraint has to be taken into account: the inertial properties of the augmented and the soft robot must be equivalent. We thus ensure that the inertial properties are equivalent by matching the centers of mass of each CC segment by an equivalent point mass in the rigid robot structure. %In this way we assure an exact equivalence of the rigid robot behavior and the soft robot, within the PCC hypothesis.
%
%This can be obtained by considering the centers of mass of each segment of the soft robot. We call a DH parametrization dynamically consistent if the modeled robot has in both representation the same amount of point masses placed at the same location, given $\xi = m(q)$. 
% For example, considering the middle point of the chord as an approximation of the CC segment center of mass, a dynamically consistent DH parametrization of the segment is described in Tab.~\ref{tab:DH2}.
Considering a point mass placed in the middle of the main chord as a suitable approximation of the mass distribution of the CC segment, a dynamically consistent DH parametrization is described in Tab.~\ref{tab:DH2}.
%, which we obtained by introducing a prismatic joint to the DH parametrization of Tab.~\ref{tab:DH1}. 
The segment map is
%
\begin{equation}\label{eq:m_ex}
	m_i(q_i) = 
	\begin{bmatrix}
		\frac{q_i}{2}\\
		L_i \frac{\sin(\frac{q_i}{2})}{q_i} \\
		L_i \frac{\sin(\frac{q_i}{2})}{q_i} \\
		\frac{q_i}{2}
	\end{bmatrix} \; .
\end{equation}

We show a graphical representation of this robot in Fig.~\ref{fig:augmented_robots_m}. A generic PCC continuous soft robot can always be matched to a dynamically consistent rigid robot, built as a sequence of these RPPR elements. We present in Fig.~\ref{fig:PCC_eq} an equivalent rigid formulation for the PCC soft robot of Fig.~\ref{fig:PCC_ex}. The robot's configurations are connected by the map %$m(q): \mathbb{R}^{\mathrm{n}} \rightarrow \mathbb{R}^{n m}$
%
\begin{equation}\label{eq:m}
	m(q) = 
    \begin{bmatrix}
		m_1(q_1)\mathrm{^T} \quad 
		\ldots \quad
		m_n(q_n)\mathrm{^T}
    \end{bmatrix}^{\mathrm{T}} \; .
\end{equation}

\begin{table}[ht]
%\normalsize
\centering 
\caption{Description of the rigid robot equivalent to a single CC segment. The parameters $\theta$, $d$, $a$, $\alpha$ refer to the classic DH parametrization, while $\mu$ refers to the mass. \label{tab:DH2}}
\begin{tabular}{cccccc}
\hline
Link &$\theta$ &d &a &$\alpha$ &$\mu$ \\
\hline
$1$      &$\dfrac{q_i}{2}$  &0                                              &0 &$\dfrac{\pi}{2}$  &0    \\
$2$      &$0$                 &$L_i \, \dfrac{\sin(\frac{q_i}{2})}{q_i}$ &0 &0 &$\mu_i$    \\
$3$      &$0$                 &$L_i \, \dfrac{\sin(\frac{q_i}{2})}{q_i}$ &0 &$-\dfrac{\pi}{2}$ &0    \\
$4$      &$\dfrac{q_i}{2}$  &0                                              &0 &$0$  &0    \\[5pt] \hline
\end{tabular}
\end{table}
%
% \begin{figure}
%     \centering
%     \subfigure[RPR]{\includegraphics[width = .47\columnwidth]{dwg/segment_dh_1}}
%     \subfigure[RPPR]{\includegraphics[width = .49\columnwidth]{dwg/segment_dh_2}}
%     \caption{Two examples of augmented robots kinematically consistent with a planar CC segment. Several of these basic elements can be connected to obtain a kinematically consistent representation of a PCC soft robot. \label{fig:augmented_robots}}
% \end{figure}

% \begin{figure}
% 	\centering
% 	\subfigure[RPPR]{\includegraphics[height = .45\columnwidth]{dwg/segment_dh}\label{fig:augmented_robots_m}}
%     \subfigure[RPRPR]{\includegraphics[height = .45\columnwidth]{dwg/segment_dh_4}}
%     \caption{Two examples of augmented robots dynamically consistent with a planar CC segment. Several of these basic elements can be connected to obtain a dynamically consistent representation of a PCC soft robot. The two structures derives from different hypotheses on the mass distribution. In (a), the center of mass is in the middle of the chord, i.e. mass concentrated at the two ends of the segment. In (b) the center of mass can be moved on the symmetry axis of the arc, e.g. implementing an homogeneous mass distribution hypothesis. \label{fig:augmented_robots_dyn}}
% \end{figure}

\begin{figure}
    \centering
    \subfigure[RPR]{\includegraphics[width = .47\columnwidth]{dwg/segment_dh_1}\label{fig:augmented_robots}}
	\subfigure[RPPR]{\includegraphics[height = .45\columnwidth]{dwg/segment_dh}\label{fig:augmented_robots_m}}
    \caption{Two examples of augmented robots kinematically consistent with a planar CC segment. Several of these basic elements can be connected to obtain a kinematically consistent representation of a PCC soft robot. 
    %
    Of the two examples only (b) takes into account the positioning of the mass of the segment, which is here placed in the middle of the chord, i.e. mass concentrated at the two ends of the segment.  \label{fig:augmented_robots_dyn}}
\end{figure}

\begin{figure}
	\centering
    \includegraphics[width = .59\columnwidth]{dwg/PCC_eq}
    \caption{Example of augmented state representation of a four segment PCC soft robot. Each segment has mass $\mu_i$ and it is actuated through a torque $\tau_i$. \label{fig:PCC_eq}}
\end{figure}

%Note however that, where not differently specified, the results presented in this section are generically valid for every dynamically consistent choice of the augmented rigid robot and map $m(q)$.

%
%
%
\subsection{Dynamics}
%
Consider the dynamics of the augmented rigid robot 
%
\begin{equation}\label{eq:xidyn}
	B_{\xi}(\xi)\ddot{\xi} + C_{\xi}(\xi,\dot{\xi})\dot{\xi} + G_{\xi}(\xi) = \tau_{\xi} + J_{\xi}^T(\xi) f_{\mathrm{ext}} \, ,
\end{equation}
%
where $\xi$, $\dot{\xi}$, $\ddot{\xi}$ is the robot configuration with its derivatives, $B_{\xi}$ is the robot's inertia matrix, $C_{\xi}\dot{\xi}$ collects Coriolis and centrifugal terms, $G_{\xi}$ takes into account the effect of gravity on the robot. %\cite{featherstone2014rigid}. 
The robot is subject to a set of control inputs $\tau_{\xi}$, and a set of external wrenches $f_{\mathrm{ext}}$, mapped through the Jacobian $J_{\xi}$. To express Eq.~\eqref{eq:xidyn} on the sub\--manifold implicitly identified by $\xi = m(q)$, we evaluate the augmented configuration derivatives $\xi$, $\dot{\xi}$, w.r.t. $q$, $\dot{q}$, $\ddot{q}$
%
\begin{equation} \label{eq:xi}
	\begin{cases}
		\xi &= m(q) \\
		\dot{\xi} &= J_{\mathrm{m}}(q) \dot{q} \\
		\ddot{\xi} &= \dot{J}_{\mathrm{m}}(q,\dot{q}) \dot{q} + J_{\mathrm{m}}(q) \ddot{q} \; .
	\end{cases}
\end{equation}
%
where $J_{\mathrm{m}}(q): \mathbb{R}^{n} \rightarrow \mathbb{R}^{n \, m \times n}$ is the Jacobian of $m(\cdot)$, defined in the usual way as $J_{\mathrm{m}} = \frac{\partial m}{\partial q}$. For example, when $m_i(q)$ is defined as in \eqref{eq:m}, the Jacobian is
%
% \begin{equation}\label{eq:Jm}
% 	\normalsize
% 	J_{\mathrm{m},i} = 
%     \begin{bmatrix}
% 		\frac{1}{2} \vspace{0.02\columnwidth}\\
% 		L_i \, \frac{q_i \, \cos(\frac{q_i}{2}) - 2 \, \sin(\frac{q_i}{2})}{2 \, q_i^2} \vspace{0.02\columnwidth} \\
% 		L_i \, \frac{q_i \, \cos(\frac{q_i}{2}) - 2 \, \sin(\frac{q_i}{2})}{2 \, q_i^2} \vspace{0.02\columnwidth}\\
% 		\frac{1}{2}
% 	\end{bmatrix}
% \end{equation}
\begin{equation}\label{eq:Jm}
	J_{\mathrm{m},i}(q_i) = 
    \begin{bmatrix}
		\frac{1}{2} \quad
		L_{c,i}(q_i) \quad
		L_{c,i}(q_i) \quad \frac{1}{2}
	\end{bmatrix}^{\mathrm{T}}
\end{equation}
where $L_{c,i}(q_i) = L_i \, \frac{q_i \, \cos(\frac{q_i}{2}) - 2 \, \sin(\frac{q_i}{2})}{2 \, q_i^2}$.
%
By substituting \eqref{eq:xi} into \eqref{eq:xidyn}, it follows
%
\begin{equation}
\begin{split}
	  B_{\xi}&(m(q)) (\dot{J}_{\mathrm{m}}(q,\dot{q}) \dot{q} + J_{\mathrm{m}}(q) \ddot{q}) \\ 
             &+ C_{\xi}(m(q),J_{\mathrm{m}}(q) \dot{q})J_{\mathrm{m}}(q) \dot{q} + G_{\xi}(m(q)) \\
             &= \tau_{\xi} + J_{\xi}^T(m(q)) f_{\mathrm{ext}} \, .
\end{split}
\end{equation}
%
%Motivated by the Operational Space formulation \cite{khatib1987unified}, 
This generalized balance of forces can be projected into the constraints through pre\-multiplication with $J_{\mathrm{m}}^{T}(q)$. This yields the compact dynamics
%
\begin{equation}\label{eq:soft_robot_dynamics}
	\begin{split}
		B(q)\ddot{q} + C(q,\dot{q})\dot{q} + G_{\mathrm{G}}(q) = \tau + J^T(q) f_{\mathrm{ext}} \, ,
	\end{split}
\end{equation}
%
where
%
\begin{equation}\label{eq:js_m_def}
	\begin{cases}
		B(q) &= J_{\mathrm{m}}^T(q) \, B_{\xi}(m(q)) \, J_{\mathrm{m}}(q) \\
		C(q,\dot{q}) &= J_{\mathrm{m}}^T(q) \, B_{\xi}(m(q)) \, \dot{J}_{\mathrm{m}}(q,\dot{q}) \\
		                    & + J_{\mathrm{m}}^T(q) \, C_{\xi}(m(q),J_{\mathrm{m}}(q) \dot{q}) \, J_{\mathrm{m}}(q) \\
		G_{\mathrm{G}}(q) &= J_{\mathrm{m}}^T(q) \, G_{\xi}(m(q))\\
		\tau &= J_{\mathrm{m}}^T(q) \, \tau_{\xi} \\
        J(q) &= J_{\xi}(m(q)) \, J_{\mathrm{m}}(q)
	\end{cases}
\end{equation}

Note that the terms in \eqref{eq:xidyn} can be efficiently formulated in an iterative form, as discussed in \cite{featherstone2014rigid}. The soft robotic model \eqref{eq:soft_robot_dynamics} inherits this property through \eqref{eq:js_m_def}. 
%Thus standard tools designed for classic rigid robots can be used \cite{corke}. %TODO: FIX citation
%
% This is a main advantage of the proposed model, 

We complete \eqref{eq:soft_robot_dynamics} by introducing linear elastic and dissipative terms. 
%(discussed in Appendix B), and a model for the input field (discussed in Appendix A). 
%
% TODO: Add nonlinear models for journal version
% TODO: Add model for input field
%
The resulting model describing the evolution of the soft robot's degree of curvature $q$ in time is
%
\begin{equation}\label{eq:soft_robot_dynamics_tot}
	B\ddot{q} + (C + D)\dot{q} + G_{\mathrm{G}} + K\,q = \tau + J^T f_{\mathrm{ext}} \, ,
\end{equation}
%
% WITH A:
%	B\ddot{q} + (C + D)\dot{q} + G_{\mathrm{G}} + K\,q = A\tau_{\mathrm{a}} + J^T f_{\mathrm{ext}} \, ,
%
where $D$ is the damping and $K$ is the stiffness.
%, and $A(q)$ is the matrix mapping control inputs $\tau_{\mathrm{a}}$ into generalized forces $\tau$. 
% As counterpart of the classic hypothesis of full actuations \cite{sciavicco2012modelling}, 
% we consider in the following $A(q)$ invertible. 
Note that the dependencies of $q,\dot{q},\ddot{q}$ were omitted for the sake of space.

% %
% % UNCOMMENT FOR THE JOURNAL VERSION
% %
% \subsection{Model properties}

% One of the main advantages of the proposed model is to verify a set of basic properties of classic rigid robots, of which we report a selection in the following. They are of great interest for the aim of the present paper, since they are used in proofs of convergence and robustness of the most commonly used control strategies in rigid robot torque control \cite{sciavicco2012modelling}. %We formulate such properties for a generic augmented formulation, underling when the result is specific for the specific considered mapping.

% \begin{Lemma}\label{Lm:C}
% 	If $C_{\xi}$ is defined with Christoffel symbols, then the matrix $B(q) - 2C(q,\dot{q})$ is skew symmetric.
% \end{Lemma}
% \begin{proof}
% 	\begin{equation}\label{eq:dB}
% 	\begin{split}
% 		\dot{B}(q) &= \dot{J}_{\mathrm{m}}^T B_{\xi} J_{\mathrm{m}} + J_{\mathrm{m}}^T \dot{B}_{\xi} J_{\mathrm{m}} + J_{\mathrm{m}}^T B_{\xi} \dot{J}_{\mathrm{m}} \\
%                    & = J_{\mathrm{m}}^T \dot{B}_{\xi} J_{\mathrm{m}} + 2 \, J_{\mathrm{m}}^T B_{\xi} \dot{J}_{\mathrm{m}} \; ,
% 	\end{split}
% \end{equation}
% %
% where in the second step we exploited the symmetry of $B_{\xi}$. Combining \eqref{eq:dB} with the expression of $C$ in \eqref{eq:js_m_def} yields to
% %
% \begin{equation}
% 	\begin{split}
% 	 \dot{B}(q) -2 \, C(q,\dot{q}) &= J_{\mathrm{m}}^T \dot{B}_{\xi} J_{\mathrm{m}} + 2 \, J_{\mathrm{m}}^T B_{\xi} \dot{J}_{\mathrm{m}}\\
%                                    &-2 J_{\mathrm{m}}^T B_{\xi} \dot{J}_{\mathrm{m}} -2 J_{\mathrm{m}}^T C_{\xi} J_{\mathrm{m}} \\
%                                    &= J_{\mathrm{m}}^T (\dot{B}_{\xi} - 2 C_{\xi}) J_{\mathrm{m}} \, .
% 	\end{split}
% \end{equation}
% %
% The proof follows by direct application of the skew symmetric definition. Indeed, for every $\nu \in \mathbb{R}^{n}$ the following holds
% %
% \begin{equation}
% 	\nu^T J_{\mathrm{m}}^T (\dot{B}_{\xi} - 2 C_{\xi}) J_{\mathrm{m}} \nu = (\nu J_{\mathrm{m}})^T (\dot{B}_{\xi} - 2 C_{\xi}) (J_{\mathrm{m}} \nu) = 0 \; ,
% \end{equation}
% %
% where in the last step we exploited the skew symmetry of $\dot{B}_{\xi} - 2 C_{\xi}$.
% \end{proof}

% \begin{Remark}
% 	If $C_{\xi}$ is not built through Christoffel symbols, the Lemma \ref{Lm:C} thesis becomes $\dot{q}^T(B(q) - 2\,(C(q,\dot{q})))\dot{q} = 0$. This can be proven by following the same steps of the current proof.
% \end{Remark}

% %
% %
% %
% \begin{Lemma}
% 	The inertia matrix $B(q)$ is positive and limited, i.e.
%     %
%     \begin{equation*}
%     	B(q) \succeq 0 \; , \quad||B(q)|| < \infty \qquad \forall q \in \mathbb{R}^n \; ,
%     \end{equation*}
%     %
%     if $- \infty < m_i(q) < + \infty$ for all $q \in \mathbb{R}^{n}$ and $i$ such that the i\--th joint is prismatic, and $||J_{\mathrm{m}}|| < \infty$.
% \end{Lemma}
% \begin{proof}
% By considering that $B_{\xi} \succeq 0$ for every $\xi$ by construction, the first property derives from the very definition of positiveness. 
% For the second property, it is sufficient to consider that $||B|| < ||J^T_{\mathrm{m}}|| \; ||B_{\xi}|| \; ||J_{\mathrm{m}}||$. The limitedness of $||B_{\xi}||$ is assured by the hypothesis on $m(q)$.
% \end{proof}

% %
% %
% %
% \begin{Remark}
% 	Both the hypotheses on $m(q)$ and on $J_{\mathrm{m}}(q)$ are verified for the representation described by \eqref{eq:m_ex}, \eqref{eq:Jm} and Tab. \ref{tab:DH2}.
% \end{Remark}

% %
% %
% %
% \begin{Remark}
% 	Note that $B_{\xi}$ is not full rank, having many massless links. So the invertibility is not assured for all possible augmented representations of the soft robot. In general the parametrization should be designed such that any of the columns of $J_{\mathrm{m}}$ is fully included in the nullspace of $B_{\xi}$. However, this property is not stringent, and it can be tested from direct evaluation. For example it is always hold by the parametrization defined by \eqref{eq:m_ex}, \eqref{eq:Jm} and Tab. \ref{tab:DH2}.
% \end{Remark}

==> 02_model21.tex <==
\section{Augmented Model Formulation}
%We first introduce the kinematics including an augmented formulation. Leveraging the augmented formulation, we describe the dynamic model and its properties.
%\subsection{Kinematics}
% \label{sec:kinematics}
We resolve the infinite dimensionality of a soft robot through the Piecewise Constant Curvature (PCC) model by considering the robot's shape as composed of a fixed number of segments with constant curvature (CC), merged such that the resulting curve is everywhere differentiable, see Fig.~\ref{fig:PCC_ex}. 
%Consider a PCC soft robot composed by $n$ CC segments. We introduce $n$ reference frames $\{S_1\},\dots,\{S_n\}$ attached at the ends of each segment, plus one base frame $\{S_0\}$.
%Fig.~\ref{fig:PCC_ex} presents an example of a soft robot composed by four CC segments.
%
%STAYS!
\begin{figure}
	\centering
    \subfigure[]{\includegraphics[height = .59\columnwidth,trim = {5 0 45 0},clip]{dwg/PCC}\label{fig:PCC_ex}} \hspace{0.005\columnwidth}
    \subfigure[]{\includegraphics[height = .59\columnwidth,trim = {5 0 45 0},clip]{dwg/PCC_eq}\label{fig:PCC_ex_eq}}
    \caption{Example of a PCC model for a soft robot, composed by four constant curvature elements. Panel (a) shows the robot kinematics. $\{S_0\}$ is the robot's base frame. A reference frame $\{S_i\}$ is attached at the end of each segment. $T_{i-1}^i$ is the homogeneous transformation mapping $\{S_{i - 1}\}$ into $\{S_i\}$. Panel (b) presents the augmented state representation of the soft robot through rigid elements. Each segment has mass $\mu_i$ and it is actuated through a torque $\tau_i$.}
\end{figure}
%
%Using the constant curvature hypothesis, ${S_{i-1}}$ and ${S_{i}}$ fully define the configuration of the $i\--th$ segment.
%
%Thus, robot kinematics can be defined by the $n$ homogeneous transformations $T_{0}^1,\dots,T_{n-1}^n$, which map each reference system to the subsequent one. 
%Without loss of generality and in the interest of conciseness, we will consider the planar case. Please refer to \cite{webster2010design} for more details about the PCC kinematics in 3D case.
%
%\begin{figure}
%  \centering
%  \includegraphics[width = .9\columnwidth,trim = {0 0 5 0},clip]{dwg/segment_c}
%  \caption{Kinematic representation of the i\--th planar constant curvature segment. Two local frames are placed at the two ends of the segment, $\{S_{i-1}\}$ and $\{S_{i}\}$ respectively. The length of the segment is $L_i$, and $q_i$ is the angle of curvature. \label{fig:CC_seg}}
%\end{figure}
%
%Fig.~\ref{fig:CC_seg} shows the kinematics of a single CC segment. 
%Under the hypothesis of non-extensibility, one variable is sufficient to describe the segment's configuration. 
We describe the relative rotation of the $i\--$th segment between the two adjacent reference systems through the configuration variable $q_i$.
%Let us call this variable $q_i$ for the $i\--$th segment, and $q \in \mathbb{R}^n$ the vector collecting $q_i$ for all the $n$ segments. Note that this angle is directly related to the segment curvature $\rho_i$ through the linear relation $q_i \, \rho_i = L_i$, where $L_i$ is the constant length of a segment. For this reason we will refer to $q_i$ as angle of curvature, or more simply as curvature.
%
% The $i\--$th homogeneous transformation is
% %can be derived using geometrical considerations as
% %
% \begin{equation} \label{eq:T}
% 	T_{i-1}^i(q_i) = 
%     \begin{bmatrix}
% 		\cos(q_i) &-\sin(q_i) &L_i\frac{\sin(q_i)}{q_i} \\
%         \sin(q_i) &\cos(q_i) &L_i\frac{1 - \cos(q_i)}{q_i} \\
%         0 &0 &1 \\
% 	\end{bmatrix} \; .
% \end{equation}
%
% Note, that for $q_i \rightarrow 0$, the transformation becomes 
% %
% \begin{equation}
% 	T_{i-1}^i(0) = \lim_{q_i \rightarrow 0}T_{i-1}^i(q_i) =
%     \begin{bmatrix}
% 		1 &0 &L_i \\
%         0 &1 &0\\
%         0 &0 &1 \\
% 	\end{bmatrix} \, .
% \end{equation}

%\subsection{Dynamics}%{Augmented Formulation}
%\label{sec:augmented}

%Eq.~\eqref{eq:T} can be reformulated using elemental Denavit-Hartenberg transformations, as described in \cite{hannan2003kinematics}. 
%
%The equivalence of both models implicitly defines a connection between the soft robot and a rigid robot described by the equivalent parametrization.  Fig.~\ref{fig:augmented_robots_dyn}, Panels (a) and (b), shows two examples of rigid robotic structures matching a single CC segment. More complex rigid structures for generic PCC soft robots can be built by interconnecting such basic elements.

We propose to describe the PCC soft robot (as e.g. Fig. \ref{fig:PCC_ex}), through an equivalent rigid robot with an augmented state space (as e.g. Fig. \ref{fig:PCC_ex_eq}). The rigid robot is such that the end points of each CC segment coincide with the correspondent reference point of the rigid robot. We also ensure that the inertial properties are equivalent by matching the centers of mass of each CC segment by an equivalent point mass in the rigid robot structure. In this way we assure an exact equivalence of the rigid robot behavior and the soft robot, within the PCC hypothesis.
%
%From a kinematic point of view, any representation satisfying the condition that the end points of each CC segment coincide with the correspondent reference points of the rigid robot is equivalent. However, as soon as we consider the dynamics of the soft and the rigid robots, another constraint has to be taken into account: the inertial properties must be equivalent. We assure that by asking that the centers of mass of each CC segment is matched by an equivalent point of mass in the rigid robot structure. 
%Fig.~\ref{fig:augmented_robots_dyn}, Panels (c) and (d), presents two examples of rigid structures dynamically matching a CC segment.

% The state space of the equivalent rigid robot is the augmented state $\xi \in \mathbb{R}^{n\,m}$, $m$ being the number of joints per CC segment and $n$ the number of segments. 
% %
% The nonlinear constraint $\xi = m(q)$ assures that the end points and the point masses of each CC segment coincide in position and orientation with the correspondent points of the rigid robot.
% %
% A generic PCC continuous soft robot can always be matched to a dynamically consistent rigid robot, built as a sequence of these elements. 


The dynamics of the augmented rigid robot is
%
\begin{equation}\label{eq:xidyn}
	B_{\xi}(\xi)\ddot{\xi} + C_{\xi}(\xi,\dot{\xi})\dot{\xi} + G_{\xi}(\xi) = J_{\xi}^T(\xi) f_{\mathrm{ext}} \, ,
\end{equation}
%
where $\xi$, $\dot{\xi}$, $\ddot{\xi} \in \mathbb{R}^{n m}$ is the robot configuration with its derivatives, $B_{\xi}\in \mathbb{R}^{n m \times n m}$ is the robot's inertia matrix, $C_{\xi}\dot{\xi}\in \mathbb{R}^{n m}$ collects Coriolis and centrifugal terms, $G_{\xi}\in \mathbb{R}^{n m}$ takes into account the effect of gravity on the robot. %\cite{featherstone2014rigid}. 
The robot is subject to a set of external wrenches $f_{\mathrm{ext}}$, mapped through the Jacobian $J_{\xi}$. 
%
We evaluate the soft robot dynamics by imposing a set of nonlinear constraints $\xi = m(q)$, assuring the above described matching between end points and the point masses. %of each CC segment coincide in position and orientation with the correspondent points of the rigid robot.
%
%To this end, we evaluate the augmented configuration derivatives $\xi$, $\dot{\xi}$, $\ddot{\xi}$, w.r.t. $q$, $\dot{q}$, $\ddot{q}$.
% %
% \begin{equation} \label{eq:xi}
% 	\begin{cases}
% 		\xi &= m(q) \\
% 		\dot{\xi} &= J_{\mathrm{m}}(q) \dot{q} \\
% 		\ddot{\xi} &= \dot{J}_{\mathrm{m}}(q,\dot{q}) \dot{q} + J_{\mathrm{m}}(q) \ddot{q} \; .
% 	\end{cases}
% \end{equation}
% %
% where $J_{\mathrm{m}}(q): \mathbb{R}^{n} \rightarrow \mathbb{R}^{n \, m \times n}$ is the Jacobian of $m(\cdot)$, i.e. $\frac{\partial m}{\partial q}$. When $m_i(q)$ is defined as in \eqref{eq:m}, it is
%
% \begin{equation}\label{eq:Jm}
% 	\normalsize
% 	J_{\mathrm{m},i} = 
%     \begin{bmatrix}
% 		\frac{1}{2} \vspace{0.02\columnwidth}\\
% 		L_i \, \frac{q_i \, \cos(\frac{q_i}{2}) - 2 \, \sin(\frac{q_i}{2})}{2 \, q_i^2} \vspace{0.02\columnwidth} \\
% 		L_i \, \frac{q_i \, \cos(\frac{q_i}{2}) - 2 \, \sin(\frac{q_i}{2})}{2 \, q_i^2} \vspace{0.02\columnwidth}\\
% 		\frac{1}{2}
% 	\end{bmatrix}
% \end{equation}
% \begin{equation}\label{eq:Jm}
% 	\normalsize
% 	J_{\mathrm{m},i} = 
%     \begin{bmatrix}
% 		\frac{1}{2} \quad
% 		L_{c,i} \quad
% 		L_{c,i} \quad \frac{1}{2}
% 	\end{bmatrix}^T
% \end{equation}
% where $L_{c,i} = L_i \, \frac{q_i \, \cos(\frac{q_i}{2}) - 2 \, \sin(\frac{q_i}{2})}{2 \, q_i^2}$.
%
%By substituting \eqref{eq:xi} into \eqref{eq:xidyn}, 
The following set of equations results
%
\begin{equation}
\begin{split}
	B_{\xi}(m(q)) (\dot{J}_{\mathrm{m}} \dot{q} + J_{\mathrm{m}} \ddot{q}) + C_{\xi}(m(q),J_{\mathrm{m}} \dot{q})J_{\mathrm{m}} \dot{q} + G_{\xi}(m(q)) \\
    = J_{\xi}^T(m(q)) f_{\mathrm{ext}} \, ,
\end{split}
\end{equation}
%
where $J_{\mathrm{m}}(q): \mathbb{R}^{n} \rightarrow \mathbb{R}^{n \, m \times n}$ is the Jacobian of $m(\cdot)$.
%
This generalized balance of forces can be projected into the constraints $\xi = m(q)$ by pre\--multiplication with $J_{\mathrm{m}}^{T}(q)$. This yields the compact dynamics
%
\begin{equation}\label{eq:soft_robot_dynamics}
	\begin{split}
		B(q)\ddot{q} + C(q,\dot{q})\dot{q} + G_{\mathrm{G}}(q) = J^T(q) f_{\mathrm{ext}} \, ,
	\end{split}
\end{equation}
%
where
%
\begin{equation}\label{eq:js_m_def}
	\begin{cases}
		B(q) &= J_{\mathrm{m}}^T(q) \, B_{\xi}(m(q)) \, J_{\mathrm{m}}(q) \\
		C(q,\dot{q}) &= J_{\mathrm{m}}^T(q) \, B_{\xi}(m(q)) \, \dot{J}_{\mathrm{m}}(q,\dot{q}) \\
		                    & + J_{\mathrm{m}}^T(q) \, C_{\xi}(m(q),J_{\mathrm{m}}(q) \dot{q}) \, J_{\mathrm{m}}(q) \\
		G_{\mathrm{G}}(q) &= J_{\mathrm{m}}^T(q) \, G_{\xi}(m(q))\\
		%\tau &= J_{\mathrm{m}}^T(q) \, \tau_{\xi} \\
        J(q) &= J_{\xi}(m(q)) \, J_{\mathrm{m}}(q)
	\end{cases}
\end{equation}
%
%Note that the terms in \eqref{eq:xidyn} can be efficiently formulated in an iterative form, as discussed in \cite{featherstone2014rigid}. The soft robotic model \eqref{eq:soft_robot_dynamics} inherits this property through \eqref{eq:js_m_def}. 

% \begin{figure}
% 	\centering
%     \includegraphics[width = 0.6\columnwidth]{dwg/segment_elastic}
%     \caption{A segment with constant curvature. An internal torque $\tau_i$ is applied at both ends. The thickness of the segment section is $2\Delta$. We consider a continuous distribution of springs and dampers. The figure shows the one connected at distance $\delta$ from the segment axis. \label{fig:segment_elastic}}
% \end{figure}
%
%
%
%
We complete \eqref{eq:soft_robot_dynamics} by introducing elastic and dissipative terms and
%(discussed in Appendix A). 
consider the soft robot actuated through a pair of internal torques for each segment.
%, see Fig.~\ref{fig:segment_elastic}. 
%The resulting mapping is the identity in the planar case.
Thus, the complete model is
%
\begin{equation}\label{eq:soft_robot_dynamics_tot}
	B(q)\ddot{q} + (C(q,\dot{q}) + D)\dot{q} + G_{\mathrm{G}}(q) + K\,q = \tau + J\mathrm{^T}(q) f_{\mathrm{ext}} \, ,
\end{equation}
%
where $D \succ 0$ is the damping and $K \succ 0$ is the stiffness.
%
%The dependencies of $q,\dot{q}$ were omitted for the sake of space.


==> 04_control.tex <==
\section{Control Design}
\label{sec:control}

In the following, we present our proposed controller design for curvature-based dynamic control and Cartesian impedance control with surface following.
%
The uncertainty introduced by the PCC and the hypothesis on the mass distribution must be properly managed by algorithms designed to be robust to model uncertainties. We thus avoid the use of complete feedback cancellations of the robot's dynamics, as well as other kinds of control actions that presented issues with robustness in classical robots, such as pre\--multiplications of feedback actions by the inverse of the inertia matrix \cite{nakanishi2008operational,sciavicco2012modelling}. 
%
% UNCOMMENT FOR THE JOURNAL VERSION
%
% \subsection{Input and output mapping}

% %
% Under these hypotheses the input mapping is implemented as 
% %
% \begin{equation}
% 	f_{\mathrm{a}} = A^{-1}(q) \, \tau \; .
% \end{equation}

%
%
%
\subsection{Curvature Dynamic Control}

We propose the following controller for implementing trajectory following in the soft robot's state space
%
\begin{equation}\label{eq:joint_space_control}
	\tau = K \bar{q} + D \dot{\bar{q}} + C(q,\dot{q})\dot{\bar{q}} + B(q)\ddot{\bar{q}} + G_{\mathrm{G}}(q) + I_{\mathrm{q}} \int (\bar{q} - q)
\end{equation}
%
where $q,\dot{q},\ddot{q}$ are the degree of curvature vector and its derivatives. $\bar{q},\dot{\bar{q}},\ddot{\bar{q}}$ are the desired evolution and its derivatives expressed in the degree of curvature space. $B$ is the robot's inertia, $C$ is the Coriolis and centrifugal matrix, $K$ and $D$ are respectively the robot's stiffness and damping matrices. The constant $I_{\mathrm{q}}$ is the gain of the integral action.

The resulting form of the closed loop system is 
%
\begin{multline}
	B(q)(\ddot{q} - \ddot{\bar{q}}) + C(q,\dot{q})(\dot{q} - \dot{\bar{q}}) - J^T(q) f_{\mathrm{ext}}\\ 
    = K (\bar{q} - q) + I_{\mathrm{q}} \int (\bar{q} - q) + D (\dot{\bar{q}} - \dot{q}) \, .
\end{multline}
%
The feed-forward action $K \bar{q} + D \dot{\bar{q}}$ is combined with the physical impedance of the system, generating a natural proportional-derivative (PD) action $K (\bar{q} - q) + D (\dot{\bar{q}} - \dot{q})$. 
%So the closed loop system resembles the one of a robot controlled through a PID controller. 
In this way the natural softness of the robot is preserved during possible interactions with an external environment. Please refer to \cite{della2017controlling} for more details on this.
%
The integral action is included for compensating the mismatches between the real system and the approximated model considered here. Note that $I_{\mathrm{q}}$ is the only parameter that needs to be tuned in the proposed algorithm, since $K$ and $D$ are defined by the physics of the system.

The stability of the closed loop can be proven through arguments similar to the ones in \cite{paden1988globally}. For the sake of space we will discuss these aspects in more detail in future extensions of this work.

%Furthermore it can be shown that in the nominal case $I_{\mathrm{q}} = 0$

%Two are the main differences w.r.t. PD+ control. First of all we consider 

%
% UNCOMMENT FOR THE JOURNAL VERSION!
%
% \begin{theo}
% 	The closed loop system defined by the controller \eqref{eq:joint_space_control} and the system \eqref{eq:soft_robot_dynamics_tot} is globally asymptotically stable w.r.t. the trajectory $(\bar{q},\dot{\bar{q}})$ if $f_{\mathrm{ext}} = 0$.
% \end{theo}
% \begin{proof}
% 	asd
    
%     PD+ controller \cite{paden1988globally}
% \end{proof}

% \begin{Corollary}\label{cr:stiff_preservation}
% 	If $\bar{q} \equiv 0$, then the equilibrium position of the closed loop system \eqref{eq:joint_space_control} \eqref{eq:soft_robot_dynamics_tot} is the same of the open loop system if $G_G(q) = 0$.
% \end{Corollary}
% \begin{proof}
	
% \end{proof}

% \begin{Remark}
% 	Corollary \ref{cr:stiff_preservation} states that the natural soft behavior is preserved in the closed loop ().
%     % get rid only of the part that we are not interested into
%     This is coherent with \cite{della2017controlling}
% \end{Remark}

% \subsection{Trajectory Tracking in operational space}

% We specify the joint space trajectory through the 

% \begin{equation}\label{eq:ik}
% 	\begin{cases}
% 		\dot{\bar{q}} &= J^+(q) (\dot{x}_{\mathrm{d}} + k(x_{\mathrm{d}} - x) \\
%         \ddot{\bar{q}} &= \dot{J}^+(q) (\dot{x}_{\mathrm{d}} + k(x_{\mathrm{d}} - x)) \\
%                        &- J^+(q)(\ddot{x}_{\mathrm{d}} + k(\dot{x}_{\mathrm{d}} - J(q) \dot{q}))
% 	\end{cases}
% \end{equation}

% discussion about the use of the measured $q$ and $x$, so to have an integral action at the end effector level \cite{sshall}



\subsection{Cartesian Impedance Control and Surface Following}

\begin{figure}
	\centering
    \includegraphics[width = .49\columnwidth,trim=0mm 0mm 0mm 0mm,clip]{dwg/ref_sys}
    \caption{The goal of the proposed Cartesian impedance controller is to simulate the presence of a spring and a damper connected between the robot's end effector and a point in space $x_{\mathrm{d}}$. The frame $(n_{\parallel},n_{\perp})$ defines the tangent and parallel directions to the environment in the contact point. \label{fig:ref_sys}}
\end{figure}

A correct regulation of the impedance at the contact point is essential to implement robust and reliable interactions with the environment. Without loss of generality, we will consider in the following as point of contact the soft robot's end effector. We define a local frame $(n_{\parallel},n_{\perp})$ connected to the end effector, as depicted in Fig.~\ref{fig:ref_sys}. The unit vector $n_{\parallel}$ is chosen to be always tangent to the environment. The unit vector $n_{\perp}$ is such that $n_{\parallel}^{\mathrm{T}} \, n_{\perp} = 0$, and always points from the inside to the outside of the environment. For the purpose of approaching, contacting, and moving along the environment, we assume the knowledge of the following information:
%
\begin{itemize}
	\item the coordinate $x_0$ of a point included within the environment
	\item the occurrence of a contact between the end effector and the environment, acquired by isInContact()
	\item parallel $n_{\parallel}$ and perpendicular $n_{\perp}$ unit vectors at the contact point, extracted by the methods {readParallelDirection()} and {readPerpendicularDirection()}, respectively
    \item the final target $x_t$ on the surface of the environment
\end{itemize}

Note that the occurrence of a contact and the contact direction can be obtained by a motion capture system or an array of force sensors mounted to the end effector.

Leveraging these knowns and the robot's dynamic model, we propose to implement the desired compliant behavior through the following dynamic feedback loop
%
\begin{equation}\label{eq:joint_space_control_2}
  \begin{split}
      \tau &= J^{\mathrm{T}}(q) (K_{\mathrm{c}} (x_{\mathrm{d}} - x) - D_{\mathrm{c}} J(q)\dot{q} ) \\
           &+ C(q,\dot{q})\dot{q} + G_{\mathrm{G}}(q) + K \, q \\
           &+ I_{\mathrm{c}} \, J^{\mathrm{T}}(q) \, n_{\parallel} \int n_{\parallel}^T (x_{\mathrm{d}} - x) \; ,
  \end{split}
\end{equation}
%
where $q,\dot{q}$ are the degree of curvature vector and its derivative. $J(q)$ is the Jacobian mapping those derivatives into the end effector velocity $\dot{x}$. $x_{\mathrm{d}}$ is a reference position for the end effector, and $x$ is the current end effector position.

%Eq. \eqref{eq:joint_space_control_2} combines three main actions. 

The term $J^{\mathrm{T}}(q) (K_{\mathrm{c}} (x_{\mathrm{d}} - x) - D_{\mathrm{c}} J(q)\dot{q} )$ simulates the presence of a spring and a damper connected between the robot's end effector and $x_{\mathrm{d}}$. This imposes the desired Cartesian impedance. $K_{\mathrm{c}}$ and $D_{\mathrm{c}}$ are the desired Cartesian stiffness and damping matrices. We choose them to be diagonal in order to implement a full decoupling within the degrees of freedom.

The elements $C(q,\dot{q})\dot{q} + G_{\mathrm{G}}(q) + K \, q$ cancel the centrifugal, Coriolis, gravitational and elastic force terms. This action is instrumental to obtain the desired decoupling at the end\--effector \cite{khatib1987unified}.
%In future work we will analyze the possibility of generating a similar behavior only by partial removal of the elastic term $K \, q$.

Finally, we introduce the integral action $ I_{\mathrm{c}} J^{\mathrm{T}}(q) n_{\parallel} \int n_{\parallel}^T (x_{\mathrm{d}} - x) $. Note that we project the error $(x_{\mathrm{d}} - x)$ on the tangent direction $n_{\parallel}$. In this way we target the goal of compensating uncertainties introduced by the proposed approximations, obtaining zero error in steady state, while avoiding generating high contact forces.

We specify the values of $x_{\mathrm{d}}$ and $n_{\parallel}$ on\--line through Algorithm~\ref{al:hl}. %, so that possible errors in the direction orthogonal to the surface are not considered in the stop condition.
%
Algorithm~\ref{al:hl} consists of two phases: approaching and exploring. In the first phase (lines 1-5), a generic point inside the environment $x_0$ is selected as reference for the impedance controller. No integral action is considered here. When the soft robot makes contact with the environment, the second phase begins (lines 6-10). Here, the desired end effector position is chosen as the final target $x_t$. A constant displacement $\delta\in\mathbb{R}^+$ in the direction $-n_{\perp}$ is manually defined to ensure maintenance of contact with the environment.
%
Algorithm~\ref{al:hl} terminates when the seminorm of the error weighted on $n_{\parallel} n_{\parallel}^T$ is under a manually defined threshold. In this way, only the error along the surface is considered.
% $|| x - x_{\mathrm{d}} ||_{n_{\parallel} n_{\parallel}^T} = \left((x - x_{\mathrm{d}})^T n_{\parallel} n_{\parallel}^T (x - x_{\mathrm{d}})\right)^{1/2}$

\begin{algorithm}%[h!]
\begin{algorithmic}[1]
\While{isInContact() == False} \Comment{Approaching}
    \State $n_{\parallel} \leftarrow [ 0 \;\; 0 ]^{\mathrm{T}} $
    \State $n_{\perp} \leftarrow [ 0 \;\; 0 ]^{\mathrm{T}} $
    \State $x_{\mathrm{d}} \leftarrow x_{0}$
\EndWhile

\While{$ || x - x_{\mathrm{d}} ||_{n_{\parallel} n_{\parallel}^T} > \epsilon $} \Comment{Exploring}
	\State $n_{\parallel} \leftarrow \mathrm{readParallelDirection()} $
    \State $n_{\perp} \leftarrow \mathrm{readPerpendicularDirection()} $
    \State $x_{\mathrm{d}} \leftarrow x_{\mathrm{t}} - n_{\perp} \delta$
\EndWhile
\end{algorithmic}
\caption{High level control \label{al:hl}}
\end{algorithm}










==> 05_simulations.tex <==
\section{Simulative results}

We implemented, tested, and evaluated the controller \eqref{eq:ik} in the absence of the design hypothesis of PCC. We considered a soft robot composed by four actuated segments of length $0.25$m. {\bf Each segment is simulated through} 

We tested the ability of Algorithm~\ref{al:hl} to efficaciously regulate the end effector position of the end effector through a static and a dynamic set of simulations.

We compared the simulated results against the benchmark state of the art in continuum soft robot manipulators. More specifically, we used the kinematic inversion algorithm in \eqref{eq:ik} with the high gain PID controller
%
\begin{equation}
	\tau = k_{\mathrm{P}} \, (\bar{q} - q) + k_{\mathrm{I}} \, \int (\bar{q} - q) + k_{\mathrm{D}} \, (\dot{\bar{q}} - \dot{q})
\end{equation}
%
The weights $k_{\mathrm{P}}$, $k_{\mathrm{I}}$, $k_{\mathrm{D}}$ were manually tuned for each task, to obtain the best of performances. This lack of versatility represents a significant limitation of the PID controller as compared to our controller. Another limitation of the PID controller is the stiffening of the robot \cite{della2017controlling}

\subsection{Set point regulation in operational space}



\subsection{Trajectory Tracking in operational space}

We consider as reference the following Lissajous curve
%
\begin{equation}
	x_d(t) =
    \begin{bmatrix}
    	0.3 \, \sin(2\,t) + 0.4 \\
        0.3 \, \cos(t) - 0.4
    \end{bmatrix} \, \mathrm{m} \, .
\end{equation}

$k_{\mathrm{P}} = 2 \, \mathrm{Nm}$, $k_{\mathrm{I}} = 1 \, \frac{\mathrm{Nm}}{\mathrm{s}}$, $k_{\mathrm{D}} = 10 \, \mathrm{Nms}$

\begin{figure}
	\centering
    \subfigure[]{\includegraphics[width = \columnwidth]{dwg/q_ev}}
    \subfigure[]{\includegraphics[width = \columnwidth]{dwg/torque_ev}}
    \caption{}
\end{figure}
%
% \begin{figure}
% 	\centering
%     \includegraphics[width = \columnwidth]{dwg/torque_ev}
%     \caption{}
% \end{figure}
%
\begin{figure}
	\centering
    \includegraphics[width = \columnwidth]{dwg/op_space_traj}
    \caption{}
\end{figure}

\subsection{Cartesian stiffness control}

==> 06_simulated_experiments.tex <==
\section{Experimental Results}
In this section, we first describe the experimental setup, followed by the experimental validation of the proposed curvature controller and the Cartesian impedance controller.

\subsection{Experimental setup}
The experimental setup used here is a modified version of a soft planar robotic arm used for kinematic motions within confined environments \cite{marchese2014whole} and autonomous object manipulation \cite{katzschmann2015autonomous}.
%
% \begin{figure}
% 	\centering
%     \includegraphics[width = \columnwidth]{dwg/comingsoon}
%     \caption{Experimental setup.}
% \end{figure}
%
The version of the soft robot used here is composed of five bidirectional segments with inflatable cavities. Each segment of the soft arm is \SI{6.3}{\cm} long. The independent pneumatic actuation of the bidirectional arm segments is achieved through an array of 10 pneumatic cylinders. The connection element between each segment is supported vertically by two ball transfers that allow the arm to move with minimal friction on a level plane.
A motion tracking system provides real-time measurements of marked points along the inextensible back of the soft arm. 
A rigid frame holds all the sub-systems together providing reliable hardware experiments without the need for camera recalibration.

\begin{figure}
	\centering
    \subfigure[Curvature]{\includegraphics[width = .925\columnwidth]{dwg/sinusoidal_evolution_I0}}
%     \caption{Evolutions of the robot's curvature during  }
% \end{figure}
%
% \begin{figure}
% 	\centering
    \subfigure[Torques]{\includegraphics[width = .925\columnwidth]{dwg/sinusoidal_evolution_I0_torques}}
    \caption{Evolutions resulting from the application of the dynamic controller \eqref{eq:joint_space_control} to the tracking of a trajectory \eqref{eq:js_tj}. The integral gain is $I_{\mathrm{q}} = 0 \frac{\mathrm{Nm}}{\mathrm{s}}$. Panel (a) shows the evolution of the degree of curvature $q$. Panel (b) presents the corresponding actuation torques. \label{fig:I0}}
\end{figure}

\begin{figure}
	\centering
    \subfigure[Curvature]{\includegraphics[width = .925\columnwidth]{dwg/sinusoidal_evolution_I08}}
%     \caption{Evolutions of the robot's curvature during  }
% \end{figure}
%
% \begin{figure}
% 	\centering
    \subfigure[Torques]{\includegraphics[width = .925\columnwidth]{dwg/sinusoidal_evolution_I08_torques}}
    \caption{Evolutions resulting from the application of the dynamic controller \eqref{eq:joint_space_control} to the tracking of a trajectory \eqref{eq:js_tj}. The integral gain is $I_{\mathrm{q}} = 0.08 \frac{\mathrm{Nm}}{\mathrm{s}}$. Panel (a) shows the evolution of the degree of curvature $q$. Panel (b) presents the corresponding actuation torques. \label{fig:I08}}
\end{figure}

\begin{figure*}
	\centering
	\subfigure[0\si{\second}]{\includegraphics[trim={6cm 0cm 14cm 3cm},clip,width = .1375\textwidth]{dwg/osc_1}}
    \subfigure[0.5\si{\second}]{\includegraphics[trim={6cm 0cm 14cm 3cm},clip,width = .1375\textwidth]{dwg/osc_2}}
    \subfigure[1\si{\second}]{\includegraphics[trim={6cm 0cm 14cm 3cm},clip,width = .1375\textwidth]{dwg/osc_3}}
    \subfigure[1.5\si{\second}]{\includegraphics[trim={6cm 0cm 14cm 3cm},clip,width = .1375\textwidth]{dwg/osc_4}}
    \subfigure[2\si{\second}]{\includegraphics[trim={6cm 0cm 14cm 3cm},clip,width = .1375\textwidth]{dwg/osc_5}}
    \subfigure[2.5\si{\second}]{\includegraphics[trim={6cm 0cm 14cm 3cm},clip,width = .1375\textwidth]{dwg/osc_6}}
    \subfigure[3\si{\second}]{\includegraphics[trim={6cm 0cm 14cm 3cm},clip,width = .1375\textwidth]{dwg/osc_7}}
    \caption{The photo sequence shows the soft robot controlled along the reference trajectory~\eqref{eq:js_tj} by the proposed curvature controller~\eqref{eq:joint_space_control}. No integral action is used here, i.e. $I_{\mathrm{q}} = 0 \frac{\mathrm{Nm}}{\mathrm{s}}$. Note that the bottom segment is not actuated and constrained in its vertical position through a mechanical stop.\label{fig:photoseq_1}}
\end{figure*}

\subsection{Identification}

The proposed model \eqref{eq:soft_robot_dynamics_tot} has several free parameters to be identified: masses $\mu_i$, lengths $L_i$, stiffnesses $k_i$, dampings $d_i$. In addition to the robot's dynamics, we also characterize the behavior of the actuators. The available inputs to our soft robot are the desired placements of the pistons within the cylinders. The placements are expressed in encoder tics, ranging from $-1000$ to $1000$ tics. We model the actuator's dynamics with a second order linear filter $\frac{\alpha_i}{(\gamma_i \, s + 1)^2}$. $\alpha_i$ and $\gamma_i$ are two additional variables to be included in the identification. The identification data were collected through three experiments. For each experiment, a step input is injected into all pneumatic cylinders. The amplitudes of the steps were $300$, $600$, and $900$ tics, respectively.

The free parameters $L_i$ and $\mu_i$ were directly measured with \SI{0.063}{\m} and \SI{0.034}{\kilo\gram}, respectively. We hypothesized the same stiffness and damping for each segment in order to reduce the search space for the identification procedure. We identified the remaining parameters by iteratively fixing $\delta_i$ to a value picked from a predefined grid. The remaining seven parameters were identified as the ones minimizing the $2\--$norm of the error between estimated and measured evolutions. For this regression problem we used the pseudo\--inverse to achieve this goal. The best performing set of parameters between all identified sets was chosen. The identified stiffness $\hat{k}$ is \SI{0.56}{\newton\meter}. The damping $\hat{d}$ is \SI{0.1066}{\newton\meter\second}. The actuator parameters are $\hat{\alpha} = 10^{-3} [0.16, \; 0.24, \; 0.2, \; 0.25, \; 0.23 ]\si{\per\newton\per\meter}$ and $\hat{\gamma} = [ 0.1, \; 0.25, \;  0.1, \;  0.1, \; 0.1]\si{\second}$.

%Remaining parameters were identified through a series of experiments performed on the robot.
%The remaining parameters were identified through the procedure described by algorithm \ref{al:Identification}.

% \begin{algorithm}%[h!]
% \begin{algorithmic}[1]
% \For{asd}
% 	\State \mathrm{Actuate the robot ang}
% \EndFor
% % \While{isInContact() == False} 
% %     \State $n_{\parallel} \leftarrow [ 0 \;\; 0 \;\; 0 ]^{\mathrm{T}} $
% %     \State $n_{\perp} \leftarrow [ 0 \;\; 0 \;\; 0 ]^{\mathrm{T}} $
% %     \State $x_{\mathrm{d}} \leftarrow x_{0}$
% % \EndWhile

% % \While{$ || x - x_{\mathrm{d}} ||_{n_{\parallel} n_{\parallel}^T} < \epsilon $} 
% % 	\State $n_{\parallel} \leftarrow \mathrm{readParallelDirection()} $
% %     \State $n_{\perp} \leftarrow \mathrm{readPerpendicularDirection()} $
% %     \State $x_{\mathrm{d}} \leftarrow x_{\mathrm{t}} - n_{\perp} \delta$
% % \EndWhile
% \end{algorithmic}
% \caption{Identification procedure \label{al:Identification}}
% \end{algorithm}

\subsection{Curvature Control}

To test the ability of the proposed curvature controller~\eqref{eq:joint_space_control}, we consider the problem of tracking the following trajectory in the degree of curvature space
%
\begin{equation}\label{eq:js_tj}
	\bar{q}_i(t) = \frac{\pi}{20} - \frac{\pi}{24}\cos(\frac{2}{3} \, \pi \, t) \quad \forall i \in \{1,\dots,5\} \, .
\end{equation}
%
%which corresponds to a total maximum required curvature of $\frac{\pi}{2}$rad, and 
%
The input to the pistons is generated by filtering $\tau$ through
%
\begin{equation} \label{eq:input_filter}
	\frac{1}{\hat{\alpha}_i}\frac{(\hat{\gamma}_i \, s + 1)^2}{(5\, T \, s + 1)^2} \, ,
\end{equation}
%
where $T=\SI{0.015}{\second}$ is the sampling time of the control system.

Fig.~\ref{fig:I0} presents the evolution of measured degrees of curvature and applied torques, with the integral action set to $I_{\mathrm{q}}=\SI{0}{\newton\meter\per\second}$. Even without any integral compensation of the model uncertainties, the algorithm is able to produce a stable oscillation close to the commanded one. The correspondent $L^2$\--norm of the error is \SI{0.1311}{\radian}. 
%
Fig.~\ref{fig:photoseq_1} presents the photo sequence of one of the resulting oscillations.

Fig.~\ref{fig:I08} shows the evolution of the same quantities for $I_{\mathrm{q}} = \SI{0.08}{\newton\meter\per\second}$. This low gain feedback appears to scarcely modify the torque profile. However this small variation reduces sensibly the tracking error, resulting in a $L^2$\--norm equal to \SI{0.0965}{\radian}. The error can be further reduced by increasing the gain to \SI{0.3}{\newton\meter\per\second}, for which the $L^2$\--norm is \SI{0.0861}{\radian}.


\subsection{Cartesian Impedance Control and Surface Following}

\begin{figure*}
	\centering
	\subfigure[]{\includegraphics[trim={6cm 0cm 14cm 0.5cm},clip,width = .16\textwidth]{dwg/cart_1_2}}
    \subfigure[]{\includegraphics[trim={6cm 0cm 14cm 0.5cm},clip,width = .16\textwidth]{dwg/cart_2_2}}
    \subfigure[]{\includegraphics[trim={6cm 0cm 14cm 0.5cm},clip,width = .16\textwidth]{dwg/cart_3_2}}
    \subfigure[]{\includegraphics[trim={6cm 0cm 14cm 0.5cm},clip,width = .16\textwidth]{dwg/cart_4_2}}
    \subfigure[]{\includegraphics[trim={6cm 0cm 14cm 0.5cm},clip,width = .16\textwidth]{dwg/cart_5_2}}
    \subfigure[]{\includegraphics[trim={6cm 0cm 14cm 0.5cm},clip,width = .16\textwidth]{dwg/cart_6_2}}
    \caption{Photo sequence of the soft robot controlled through the proposed Cartesian impedance controller \eqref{eq:joint_space_control_2}. We report superimposed the two reference positions commanded by Algorithm~\ref{al:hl} (red crosses) and the trajectory of the end effector (blue dashed line). Panels (a-c) show the first phase of the algorithm: the robot's tip is attracted toward the environment by a virtual spring connected to a reference point inside the surface. Panels (d-f) illustrate the second phase of the algorithm: the robot traces along the surface toward the desired end position. Note that the bottom segment is not actuated and constrained in its vertical position through a mechanical stop. \label{fig:photoseq_2}}
    \vspace{-5pt}
\end{figure*}

\begin{figure}
	\centering
	\includegraphics[width = \columnwidth]{dwg/cartesian_torque}
    \caption{Actuation torques commanded by the proposed Cartesian impedance controller \eqref{eq:joint_space_control_2} while executing the Algorithm \ref{al:hl}. The contact detection happens at \SI{6.5}{\second}. \label{fig:cartesian_torque}}
\end{figure}
%
\begin{figure}
	\centering
	\includegraphics[width = \columnwidth]{dwg/certesian_ee.eps}
    \caption{End effector's evolution in Cartesian space resulting by the application of the proposed Cartesian impedance controller \eqref{eq:joint_space_control_2} and Algorithm \ref{al:hl}. The contact detection happens at \SI{6.5}{\second}. \label{fig:cartesian_ee}}
\end{figure}

We test the effectiveness of the proposed Cartesian impedance controller and surface following strategy. The robot's goal is to first reach the wall and then slide along it until the desired position is reached. Note that we are not interested in a precise regulation of the contact forces. Instead, the constraint imposed by the environment is purposefully exploited in combination with the decoupled compliance imposed by the control, to naturally generate the interaction forces and guide the end effector toward the desired position.

The input to the pneumatic cylinders is produced by filtering $\tau$ in \eqref{eq:joint_space_control_2} through the filter described in \eqref{eq:input_filter}. The desired impedance at the end effector is
%
\begin{equation}
	K_{\mathrm{c}} = \begin{bmatrix}
		13 &0\\
        0 &13
	\end{bmatrix}\si{\newton\meter\per\radian} \quad 
    D_{\mathrm{c}} = \begin{bmatrix}
		6 &0\\
        0 &6
	\end{bmatrix}\si{\newton\meter\second\per\radian} \; .
\end{equation}
%
The integral gain is $I_c = 1.9 \si{\newton\meter\per\radian\per\second}$. 
%

As described in Algorithm~\ref{al:hl}, the experiment is divided in two phases. In the first one, the end effector of the soft robot is attracted toward a point within the environment ($x_0 = [0.283, 0.135]\si{\meter}$), which is manually defined.  

After contact is established, it triggers the execution of the second phase. The end-effector is now pulled towards a new target ($x_{\mathrm{d}} = [0.220, 0.160]$\si{\meter}) while staying in contact. The distance to the wall is maintained with $\delta = 0.05$\si{\meter}. The values of $n_{\perp}$ and $n_{\parallel}$ are considered known.

For one example experiment, the commanded actuation torques are shown in Fig.~\ref{fig:cartesian_torque}. The evolution of the end effector in Cartesian space is shown in Fig.~\ref{fig:cartesian_ee}, while the correspondent photo sequence is shown in Fig.~\ref{fig:photoseq_2}.

==> 07_conclusion.tex <==
% \section{Discussion}
% \subsection{Limitations}
% What we don't have, and it would be good to have in the paper
% \begin{enumerate}
% \item Feedback controller working on Simscape simulator (or in either cases, more extensive simulations)
% \item augmenting the xi space placing the mass in the actual center of mass of the segment
% \item implementing the tracking at the end effector (instead of the regulation)
% \end{enumerate}
\section{Conclusion}
%
In this paper we present two new algorithms that achieve dynamic control of soft robots and enable interactions between soft robots and their environment. Both algorithms leverage on the idea of connecting the soft robot to an equivalent augmented rigid robot, in such a way that the matching is exact in the common hypothesis of constant curvature, and under the introduced hypothesis on the mass distribution. Classic tools in robotic control are used to develop robust feedback control strategies able to compensate for any model mismatch. We implement the control algorithms on a planar multi-link soft robotic manipulator and demonstrate curvature control and surface following using our strategy.  

The control algorithm presented in this paper has been evaluated in the context of exploring a two-dimensional surface using a soft planar robot manipulator. However, the potential for this work is much broader. 
%The algorithm has been inspired by nature, specifically by the way in which elephants use their soft trunks to explore the world. 
The control algorithm is general and has the potential to enable a wide range of dynamic tasks, ranging from exploring three dimensional spaces through contact, learning the geometry of the world, picking up delicate objects, moving heavy objects and enabling dynamic interactions with the world. 

% TODO: Describe:
% Non-linear elastic and dissipative model
% Input Model A

% \subsection{Future work} 
% \begin{enumerate}
% \item 3D case (more clever parametrization)
% \item more exciting simulations (with an actual "smell field", that I would not discuss here)
% \item dynamic control for limited torque
% \item design and realization of a robotic trunk
% \item experiments with the new robot
% \end{enumerate}



